Offline Handwritten Signature Verification Using a Stream-Based Approach

Handwritten Signature Verification (HSV) systems distinguish between genuine and forged signatures. Traditional HSV development involves a static batch configuration, constraining the system's ability to model signatures to the limited data available. Signatures exhibit high intra-class variability and are sensitive to various factors, including time and external influences, imparting them a dynamic nature. This paper investigates the signature learning process within a data stream context. We propose a novel HSV approach with an adaptive system that receives an infinite sequence of signatures and is updated over time. Experiments were carried out on GPDS Synthetic, CEDAR, and MCYT datasets. Results demonstrate the superior performance of the proposed method compared to standard approaches that use a Support Vector Machine as a classifier. Implementation of the method is available at https://github.com/kdMoura/stream_hsv.

==> figures/fig_stream_sgd_svm_cedar_mcyt_mixed/pdf/main_pdf.tex <==
\begin{figure}[H]
    \centering
    
    %\textbf{CEDAR and MCYT randomly | skilled | 10 ref(s) | G = 12}
    
    %\vspace{-4cm}
    
    % First row of charts
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{figures/fig_stream_sgd_svm_cedar_mcyt_mixed/fig_stream_sgd_svm_r10_ch200_u5_g12_tr_sgpds_signets_ts_cedar_mcyt_mixed_skilled_global_eer.pdf}
        \caption{\#Users ($n\mathcal{D}$) = 5, \#G sig = 12}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{figures/fig_stream_sgd_svm_cedar_mcyt_mixed/fig_stream_sgd_svm_r10_ch200_u10_g12_tr_sgpds_signets_ts_cedar_mcyt_mixed_skilled_global_eer.pdf}
        \caption{\#Users ($n\mathcal{D}$) = 10, \#G sig = 12}
    \end{subfigure}
    
    % Second row of charts
    \vspace{0.1cm} % Adjust vertical space between rows
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{figures/fig_stream_sgd_svm_cedar_mcyt_mixed/fig_stream_sgd_svm_r10_ch200_u50_g12_tr_sgpds_signets_ts_cedar_mcyt_mixed_skilled_global_eer.pdf}
        \caption{\#Users ($n\mathcal{D}$) = 50, \#G sig = 12}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{figures/fig_stream_sgd_svm_cedar_mcyt_mixed/fig_stream_sgd_svm_r10_ch200_uall_g12_tr_sgpds_signets_ts_cedar_mcyt_mixed_skilled_global_eer.pdf}
        \caption{\#Users ($n\mathcal{D}$) = All, \#G sig = 12}
    \end{subfigure}
    
    % Third row for the legend
    \vspace{0.1cm} % Adjust vertical space for the legend
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\linewidth, trim=2cm 0cm 1cm 14cm, clip]{figures/fig_stream_sgd_svm_cedar_mcyt_mixed/fig_stream_sgd_svm_other_streams_legend}
    \end{subfigure}
    
    \caption{Stream evaluation of skilled forgery detection on signatures randomly coming from the CEDAR and MCYT streams using SVM and the Stream HSV (SHSV). The evaluation considers 10 reference signatures with a Max fusion for decision-making. SHSV is updated after every training chunk and evaluated on every window (Table~\ref{tab:stream_evaluation}). \#Users ($n\mathcal{D}$) and \#G denote the number of users and genuine signatures used in the initial training. }
    \label{fig:stream_svm_sgd_r10_ch200_g12_tr_sgpds_signets_ts_cedar_mcyt_mixed_skilled_global}
\end{figure}

    
